Shape-from-intrinsic operator

Shape-from-X is an important class of problems in the fields of geometry processing, computer graphics, and vision, attempting to recover the structure of a shape from some observations. In this paper, we formulate the problem of shape-from-operator (SfO), recovering an embedding of a mesh from intrinsic differential operators defined on the mesh. Particularly interesting instances of our SfO problem include synthesis of shape analogies, shape-from-Laplacian reconstruction, and shape exaggeration. Numerically, we approach the SfO problem by splitting it into two optimization sub-problems that are applied in an alternating scheme: metric-from-operator (reconstruction of the discrete metric from the intrinsic operator) and embedding-from-metric (finding a shape embedding that would realize a given metric, a setting of the multidimensional scaling problem).

==> sections/fig_hands_negativeweigths.tex <==
%
%
%\begin{figure}[htbp]
%\centering
%%
%\begin{minipage}{\columnwidth}
%	%
%	\begin{overpic}
%	% trim={<left> <lower> <right> <upper>}
%	[trim={4cm 0cm 0cm 0cm},clip,width=0.4\textwidth]{./figures/hands_negativeweights/hands_to_original_negativeweights.eps}
%	\end{overpic}
%	%
%	\begin{overpic}
%	[trim={4cm 0cm 0cm 0cm},clip,width=0.4\textwidth]{./figures/hands_negativeweights/hand_to_remesh_negativeweights.eps}
%	\end{overpic} 
%	%
%\end{minipage}
%%
%\end{figure}


\begin{figure}[htbp]
\centering
%
\begin{minipage}{0.8\columnwidth}
	\begin{overpic}
	% trim={<left> <lower> <right> <upper>}
	[trim={0cm 0cm 0cm 0cm},clip,width=\textwidth]{./figures/hands_negativeweights/hands_negativeweights.eps}
	\end{overpic}
\end{minipage}
\caption{A shape with bad triangulation (left) results in a Laplacian with many negative weights (highlighted in red). With a more regular triangulation such as the one generated with isotropic remeshing, the number of negative weights is drastically reduced. }
\label{fig:remeshing}
\end{figure}
	
